Video Mamba Suite: State Space Model as a Versatile Alternative for Video Understanding

Understanding videos is one of the fundamental directions in computer vision research, with extensive efforts dedicated to exploring various architectures such as RNN, 3D CNN, and Transformers. The newly proposed architecture of state space model, e.g., Mamba, shows promising traits to extend its success in long sequence modeling to video modeling. To assess whether Mamba can be a viable alternative to Transformers in the video understanding domain, in this work, we conduct a comprehensive set of studies, probing different roles Mamba can play in modeling videos, while investigating diverse tasks where Mamba could exhibit superiority. We categorize Mamba into four roles for modeling videos, deriving a Video Mamba Suite composed of 14 models/modules, and evaluating them on 12 video understanding tasks. Our extensive experiments reveal the strong potential of Mamba on both video-only and video-language tasks while showing promising efficiency-performance trade-offs. We hope this work could provide valuable data points and insights for future research on video understanding. Code is public: https://github.com/OpenGVLab/video-mamba-suite.

==> sections/0_abstract_pub.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{imgs/suite.pdf}
%     \vspace{-1.5em}
%     \caption{We investigate SSMs exemplified by Mamba on video understanding. Our \texttt{Video Mamba Suite} comprises 14 SSM models/modules for 12 video understanding tasks. We explore 4 roles of SSM in video modeling and conduct extensive experiments on 13 major datasets.}
%     \label{fig:suite}
%     \vspace{-2em}
% \end{figure}




\vspace{-1.5em}
\begin{abstract}
Understanding videos is one of the fundamental directions in computer vision research, with extensive efforts dedicated to exploring various architectures such as RNN, 3D CNN, and Transformers. 
The newly proposed architecture of state space model, \textit{e.g.}, Mamba, shows promising traits to extend its success in long sequence modeling to video modeling. 
To assess whether Mamba can be a viable alternative to Transformers in the video understanding domain, in this work, we conduct a comprehensive set of studies, probing different roles Mamba can play in modeling videos, while investigating diverse tasks where Mamba could exhibit superiority. 
We categorize Mamba into four roles for modeling videos, deriving a \texttt{Video Mamba Suite}\charimage{example-image} composed of 14 models/modules, and evaluating them on 12 video understanding tasks. Our extensive experiments reveal the strong potential of Mamba on both video-only and video-language tasks while showing promising efficiency-performance trade-offs.
We hope this work could provide valuable data points and insights for future research on video understanding. Code is public: \textbf{\url{https://github.com/OpenGVLab/video-mamba-suite}.}
% \keywords{Video Understanding \and State Space Model \and Mamba}
\end{abstract}
